Which Channel to Ask My Question? Personalized Customer Service Request Stream Routing using Deep Reinforcement Learning

Customer services are critical to all companies, as they may directly connect to the brand reputation. Due to a great number of customers, e-commerce companies often employ multiple communication channels to answer customers' questions, for example, chatbot and hotline. On one hand, each channel has limited capacity to respond to customers' requests, on the other hand, customers have different preferences over these channels. The current production systems are mainly built based on business rules, which merely considers tradeoffs between resources and customers' satisfaction. To achieve the optimal tradeoff between resources and customers' satisfaction, we propose a new framework based on deep reinforcement learning, which directly takes both resources and user model into account. In addition to the framework, we also propose a new deep-reinforcement-learning based routing method-double dueling deep Q-learning with prioritized experience replay (PER-DoDDQN). We evaluate our proposed framework and method using both synthetic and a real customer service log data from a large financial technology company. We show that our proposed deep-reinforcement-learning based framework is superior to the existing production system. Moreover, we also show our proposed PER-DoDDQN is better than all other deep Q-learning variants in practice, which provides a more optimal routing plan. These observations suggest that our proposed method can seek the trade-off where both channel resources and customers' satisfaction are optimal.

==> references.tex <==
\begin{thebibliography}{100}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{Avissar:2002:OMA:581888.581891}
O.~Avissar, R.~Barua, and D.~Stewart, ``An optimal memory allocation scheme for
  scratch-pad-based embedded systems,'' \emph{ACM Trans. Embed. Comput. Syst.},
  vol.~1, no.~1, pp. 6--26, 2002.

\bibitem{Rao:2009:VRL:1555228.1555263}
J.~Rao, X.~Bu, C.-Z. Xu, L.~Wang, and G.~Yin, ``Vconf: A reinforcement learning
  approach to virtual machines auto-configuration,'' in \emph{Proc. ICAC},
  2009, pp. 137--146.

\bibitem{DBLP:journals/cor/CormanDPP14}
F.~Corman, A.~D'Ariano, D.~Pacciarelli, and M.~Pranzo, ``Dispatching and
  coordination in multi-area railway traffic management,'' \emph{Computers {\&}
  {OR}}, vol.~44, pp. 146--160, 2014.

\bibitem{Sidi:1990:CRP:647413.725039}
M.~Sidi and H.~Levy, ``Customer routing on polling systems,'' in \emph{Proc.
  Performance}, 1990, pp. 319--331.

\bibitem{wiki:RMSE}
\BIBentryALTinterwordspacing
Wikipedia, ``Rmse,'' 2018, [Online; accessed 5 November 2018, at 16:30 (UTC)].
  [Online]. Available:
  \url{https://en.wikipedia.org/wiki/Root-mean-square_deviation}
\BIBentrySTDinterwordspacing

\bibitem{wiki:RL-intro}
\BIBentryALTinterwordspacing
------, ``Reinforcement learning,'' 2018, [Online; accessed 2 October 2018, at
  17:42 (UTC)]. [Online]. Available:
  \url{https://en.wikipedia.org/wiki/Reinforcement_learning}
\BIBentrySTDinterwordspacing

\bibitem{DBLP:RL_def}
R.~Marcus and O.~Papaemmanouil, ``Deep reinforcement learning for join order
  enumeration,'' \emph{CoRR}, vol. abs/1803.00055, 2018.

\bibitem{Watkins:1989}
C.~J. C.~H. Watkins, ``Learning from delayed rewards,'' Ph.D. dissertation,
  King's College, Cambridge, UK, May 1989.

\bibitem{DBLP:journals/corr/HosuR16}
I.-A. Hosu and T.~Rebedea, ``Playing atari games with deep reinforcement
  learning and human checkpoint replay,'' \emph{CoRR}, vol. abs/1607.05077,
  2016.

\bibitem{DBLP:journals/nature/MnihKSRVBGRFOPB15}
V.~Mnih, K.~Kavukcuoglu, D.~Silver, A.~A. Rusu, J.~Veness, M.~G. Bellemare,
  A.~Graves, M.~A. Riedmiller, A.~Fidjeland, G.~Ostrovski, S.~Petersen,
  C.~Beattie, A.~Sadik, I.~Antonoglou, H.~King, D.~Kumaran, D.~Wierstra,
  S.~Legg, and D.~Hassabis, ``Human-level control through deep reinforcement
  learning,'' \emph{Nature}, vol. 518, no. 7540, pp. 529--533, 2015.

\bibitem{DBLP:conf/aaai/HasseltGS16}
H.~van Hasselt, A.~Guez, and D.~Silver, ``Deep reinforcement learning with
  double {Q}-learning,'' in \emph{Proc. AAAI}, 2016, pp. 2094--2100.

\bibitem{DBLP:journals/corr/SchaulQAS15}
T.~Schaul, J.~Quan, I.~Antonoglou, and D.~Silver, ``Prioritized experience
  replay,'' \emph{CoRR}, vol. abs/1511.05952, 2015.

\bibitem{DBLP:conf/icml/WangSHHLF16}
Z.~Wang, T.~Schaul, M.~Hessel, H.~van Hasselt, M.~Lanctot, and N.~de~Freitas,
  ``Dueling network architectures for deep reinforcement learning,'' in
  \emph{Proc. ICML}, 2016, pp. 1995--2003.

\bibitem{DBLP:journals/corr/LevineFDA15}
\BIBentryALTinterwordspacing
S.~Levine, C.~Finn, T.~Darrell, and P.~Abbeel, ``End-to-end training of deep
  visuomotor policies,'' \emph{CoRR}, vol. abs/1504.00702, 2015. [Online].
  Available: \url{http://arxiv.org/abs/1504.00702}
\BIBentrySTDinterwordspacing

\bibitem{Sutton+Barto:2018}
R.~S. Sutton and A.~G. Barto, \emph{Reinforcement Learning: An
  Introduction}.\hskip 1em plus 0.5em minus 0.4em\relax MIT Press, 2018.

\bibitem{DBLP:first-come-first-serve}
R.~Zhang and M.~Pavone, ``Control of robotic mobility-on-demand systems: a
  queueing-theoretical perspective,'' \emph{Int. J. Robotics Res}, vol.~35, no.
  1-3, pp. 186--203, 2016.

\bibitem{DBLP:conf/wkdd/TangRTC10}
\BIBentryALTinterwordspacing
M.~Tang, E.~Ren, Z.~Tang, and B.~Chen, ``Transit vehicle dispatching based on
  genetic algorithm-rbf neural network,'' in \emph{Third International
  Conference on Knowledge Discovery and Data Mining, {WKDD} 2010, Phuket,
  Thailand, 9-10 January 2010}, 2010, pp. 108--110. [Online]. Available:
  \url{https://doi.org/10.1109/WKDD.2010.58}
\BIBentrySTDinterwordspacing

\bibitem{DBLP:conf/gca/NedunchelianKMR06}
R.~Nedunchelian, K.~Koushik, M.~Nagappan, and V.~Raghu, ``Dynamic task
  scheduling using parallel genetic algorithms for heterogeneous distributed
  computing,'' in \emph{Proc. GCA}, 2006, pp. 82--88.

\bibitem{Zhou2010Synthetically}
L.~Zhou and H.~Hui, ``Synthetically improved genetic algorithm in public
  traffic dispatch system,'' in \emph{Proc. ICMLC}, 2010, pp. 5169--5172.

\bibitem{rght-kdd17}
K.~Ristovski, C.~Gupta, K.~Harada, and H.~Tang, ``Dispatch with confidence:
  {I}ntegration of machine learning, optimization and simulation for open pit
  mines,'' in \emph{Proc. KDD}, 2017, pp. 1981--1989.

\bibitem{Xu:2018:LOD:3219819.3219824}
Z.~Xu, Z.~Li, Q.~Guan, D.~Zhang, Q.~Li, J.~Nan, C.~Liu, W.~Bian, and J.~Ye,
  ``Large-scale order dispatch in on-demand ride-hailing platforms: A learning
  and planning approach,'' in \emph{Proc. KDD}, 2018, pp. 905--913.

\bibitem{DBLP:journals/corr/abs-1302-6613}
\BIBentryALTinterwordspacing
R.~Adhikari and R.~K. Agrawal, ``An introductory study on time series modeling
  and forecasting,'' \emph{CoRR}, vol. abs/1302.6613, 2013. [Online].
  Available: \url{http://arxiv.org/abs/1302.6613}
\BIBentrySTDinterwordspacing

\bibitem{wiki:Timeseries-def}
\BIBentryALTinterwordspacing
Wikipedia, ``Time series,'' 2018, [Online; accessed 28 October 2018, at 19:49
  (UTC).]. [Online]. Available: \url{https://en.wikipedia.org/wiki/Time_series}
\BIBentrySTDinterwordspacing

\bibitem{DBLP:conf/uksim/AriyoAA14}
A.~A. Ariyo, A.~O. Adewumi, and C.~K. Ayo, ``Stock price prediction using the
  {ARIMA} model,'' in \emph{Proc. UKSim}, 2014, pp. 106--112.

\bibitem{manual:LOA}
S.~S. P.~Andreea-Cristina and A.~Tindeche, ``Limitation of arima models in
  financial and monetary economics,'' \emph{J. TAE}, pp. 19--42, 2016.

\bibitem{DBLP:journals/corr/SakSB14}
H.~Sak, A.~Senior, and F.~Beaufays, ``Long short-term memory recurrent neural
  network architectures for large scale acoustic modeling,'' in \emph{Proc.
  INTERSPEECH}, 2014, pp. 338--342.

\bibitem{Gers01longshort-term}
F.~Gers, ``Long short-term memory in recurrent neural networks,'' 2001.

\bibitem{DBLP:journals/corr/AzzouniP17}
\BIBentryALTinterwordspacing
A.~Azzouni and G.~Pujolle, ``A long short-term memory recurrent neural network
  framework for network traffic matrix prediction,'' \emph{CoRR}, vol.
  abs/1705.05690, 2017. [Online]. Available:
  \url{http://arxiv.org/abs/1705.05690}
\BIBentrySTDinterwordspacing

\bibitem{DBLP:conf/icann/GersES01}
F.~A. Gers, D.~Eck, and J.~Schmidhuber, ``Applying {LSTM} to time series
  predictable through time-window approaches,'' in \emph{Proc. ICANN}, 2001,
  pp. 669--676.

\bibitem{DBLP:journals/ml/Breiman01}
L.~Breiman, ``Random forests,'' \emph{Machine Learning}, vol.~45, no.~1, pp.
  5--32, 2001.

\bibitem{DBLP:journals/eswa/LinWXZ17}
L.~Lin, F.~Wang, X.~Xie, and S.~Zhong, ``Random forests-based extreme learning
  machine ensemble for multi-regime time series prediction,'' \emph{Expert
  Syst. Appl.}, vol.~83, pp. 164--176, 2017.

\bibitem{CIS-323484}
J.~H. Friedman, ``Greedy function approximation: A gradient boosting machine.''
  \emph{The Annals of Statistics}, vol.~29, no.~5, pp. 1189--1232, 2001.

\bibitem{su8111100}
\BIBentryALTinterwordspacing
C.~Ding, D.~Wang, X.~Ma, and H.~Li, ``Predicting short-term subway ridership
  and prioritizing its influential factors using gradient boosting decision
  trees,'' \emph{Sustainability}, vol.~8, no.~11, 2016. [Online]. Available:
  \url{http://www.mdpi.com/2071-1050/8/11/1100}
\BIBentrySTDinterwordspacing

\bibitem{Friedman:2002:SGB:635939.635941}
\BIBentryALTinterwordspacing
J.~H. Friedman, ``Stochastic gradient boosting,'' \emph{Comput. Stat. Data
  Anal.}, vol.~38, no.~4, pp. 367--378, Feb. 2002. [Online]. Available:
  \url{http://dx.doi.org/10.1016/S0167-9473(01)00065-2}
\BIBentrySTDinterwordspacing

\bibitem{7514015}
G.~Barta, G.~Nagy, G.~Papp, and G.~Simon, ``Forecasting framework for open
  access time series in energy,'' in \emph{2016 IEEE International Energy
  Conference (ENERGYCON)}, April 2016, pp. 1--6.

\bibitem{DBLP:journals/ijgi/ZhangZHGCL16}
F.~Zhang, X.~Zhu, T.~Hu, W.~Guo, C.~Chen, and L.~Liu, ``Urban link travel time
  prediction based on a gradient boosting method considering spatiotemporal
  correlations,'' \emph{Int. J. Geo-Information}, vol.~5, no.~11, p. 201, 2016.

\bibitem{DBLP:journals/corr/ChenG16}
T.~Chen and C.~Guestrin, ``{XGBoost}: {A} scalable tree boosting system,''
  \emph{CoRR}, vol. abs/1603.02754, 2016.

\bibitem{wang2017electricity}
W.~Wang, Y.~Shi, G.~Lyn, and W.~Deng, ``Electricity consumption prediction
  using xgboost based on discrete wavelet transform,'' \emph{DEStech Trans. on
  Comp. Sci. and Eng.}, no. aiea, 2017.

\bibitem{DBLP:journals/corr/KingmaB14}
\BIBentryALTinterwordspacing
D.~P. Kingma and J.~Ba, ``Adam: {A} method for stochastic optimization,''
  \emph{CoRR}, vol. abs/1412.6980, 2014. [Online]. Available:
  \url{http://arxiv.org/abs/1412.6980}
\BIBentrySTDinterwordspacing

\bibitem{DBLP:journals/corr/abs-1710-02298}
\BIBentryALTinterwordspacing
M.~Hessel, J.~Modayil, H.~van Hasselt, T.~Schaul, G.~Ostrovski, W.~Dabney,
  D.~Horgan, B.~Piot, M.~G. Azar, and D.~Silver, ``Rainbow: Combining
  improvements in deep reinforcement learning,'' \emph{CoRR}, vol.
  abs/1710.02298, 2017. [Online]. Available:
  \url{http://arxiv.org/abs/1710.02298}
\BIBentrySTDinterwordspacing

\bibitem{martinetz1993neural}
T.~M. Martinetz, S.~G. Berkovich, K.~J. Schulten \emph{et~al.},
  ``{``Neural-gas''} network for vector quantization and its application to
  time-series prediction,'' \emph{IEEE. Trans. Neural Networks}, vol.~4, no.~4,
  pp. 558--569, 1993.

\bibitem{DBLP:conf/icml/WunderLB10}
M.~Wunder, M.~L. Littman, and M.~Babes, ``Classes of multiagent q-learning
  dynamics with epsilon-greedy exploration,'' in \emph{Proc. ICML}, 2010, pp.
  1167--1174.

\bibitem{nowok2016synthpop}
B.~Nowok, G.~M. Raab, C.~Dibben \emph{et~al.}, ``synthpop: Bespoke creation of
  synthetic data in r,'' \emph{J. Stat. Softw}, vol.~74, no.~11, pp. 1--26,
  2016.

\bibitem{Laptev2017TimeseriesEE}
N.~Laptev, J.~Yosinski, L.~E. Li, and S.~Smyl, ``Time-series extreme event
  forecasting with neural networks at uber,'' in \emph{Proc. ICML}, 2017, pp.
  1--5.

\bibitem{DBLP:journals/wc/MaoTFKAIM18}
\BIBentryALTinterwordspacing
B.~Mao, F.~Tang, Z.~M. Fadlullah, N.~Kato, O.~Akashi, T.~Inoue, and
  K.~Mizutani, ``A novel non-supervised deep-learning-based network traffic
  control method for software defined wireless networks,'' \emph{{IEEE}
  Wireless Commun.}, vol.~25, no.~4, pp. 74--81, 2018. [Online]. Available:
  \url{https://doi.org/10.1109/MWC.2018.1700417}
\BIBentrySTDinterwordspacing

\bibitem{DBLP:journals/tvt/MaYCG19}
\BIBentryALTinterwordspacing
Z.~Ma, H.~Yu, W.~Chen, and J.~Guo, ``Short utterance based speech language
  identification in intelligent vehicles with time-scale modifications and deep
  bottleneck features,'' \emph{{IEEE} Trans. Vehicular Technology}, vol.~68,
  no.~1, pp. 121--128, 2019. [Online]. Available:
  \url{https://doi.org/10.1109/TVT.2018.2879361}
\BIBentrySTDinterwordspacing

\bibitem{DBLP:journals/corr/abs-1712-05929}
\BIBentryALTinterwordspacing
J.~Wang, J.~Wang, Y.~Wu, J.~Wang, H.~Zhu, M.~Lin, and J.~Wang, ``A machine
  learning framework for resource allocation assisted by cloud computing,''
  \emph{CoRR}, vol. abs/1712.05929, 2017. [Online]. Available:
  \url{http://arxiv.org/abs/1712.05929}
\BIBentrySTDinterwordspacing

\bibitem{DBLP:journals/tgrs/ChengZH16}
\BIBentryALTinterwordspacing
G.~Cheng, P.~Zhou, and J.~Han, ``Learning rotation-invariant convolutional
  neural networks for object detection in {VHR} optical remote sensing
  images,'' \emph{{IEEE} Trans. Geoscience and Remote Sensing}, vol.~54,
  no.~12, pp. 7405--7415, 2016. [Online]. Available:
  \url{https://doi.org/10.1109/TGRS.2016.2601622}
\BIBentrySTDinterwordspacing

\bibitem{DBLP:journals/tcsv/HanZH0RW15}
\BIBentryALTinterwordspacing
J.~Han, D.~Zhang, X.~Hu, L.~Guo, J.~Ren, and F.~Wu, ``Background prior-based
  salient object detection via deep reconstruction residual,'' \emph{{IEEE}
  Trans. Circuits Syst. Video Techn.}, vol.~25, no.~8, pp. 1309--1321, 2015.
  [Online]. Available: \url{https://doi.org/10.1109/TCSVT.2014.2381471}
\BIBentrySTDinterwordspacing

\bibitem{DBLP:journals/ijcv/ZhangHLWL16}
\BIBentryALTinterwordspacing
D.~Zhang, J.~Han, C.~Li, J.~Wang, and X.~Li, ``Detection of co-salient objects
  by looking deep and wide,'' \emph{International Journal of Computer Vision},
  vol. 120, no.~2, pp. 215--232, 2016. [Online]. Available:
  \url{https://doi.org/10.1007/s11263-016-0907-4}
\BIBentrySTDinterwordspacing

\bibitem{DBLP:journals/pami/ZhangMH17}
\BIBentryALTinterwordspacing
D.~Zhang, D.~Meng, and J.~Han, ``Co-saliency detection via a self-paced
  multiple-instance learning framework,'' \emph{{IEEE} Trans. Pattern Anal.
  Mach. Intell.}, vol.~39, no.~5, pp. 865--878, 2017. [Online]. Available:
  \url{https://doi.org/10.1109/TPAMI.2016.2567393}
\BIBentrySTDinterwordspacing

\bibitem{DBLP:journals/access/SiYM16}
\BIBentryALTinterwordspacing
Z.~Si, H.~Yu, and Z.~Ma, ``Learning deep features for {DNA} methylation data
  analysis,'' \emph{{IEEE} Access}, vol.~4, pp. 2732--2737, 2016. [Online].
  Available: \url{https://doi.org/10.1109/ACCESS.2016.2576598}
\BIBentrySTDinterwordspacing

\bibitem{8643866}
D.~{Hu}, S.~{Zhou}, Q.~{Shen}, S.~{Zheng}, Z.~{Zhao}, and Y.~{Fan}, ``Digital
  image steganalysis based on visual attention and deep reinforcement
  learning,'' \emph{IEEE Access}, pp. 1--1, 2019.

\bibitem{8329419}
D.~{Zhang}, L.~{Qian}, B.~{Mao}, C.~{Huang}, B.~{Huang}, and Y.~{Si}, ``A
  data-driven design for fault detection of wind turbines using random forests
  and xgboost,'' \emph{IEEE Access}, vol.~6, pp. 21\,020--21\,031, 2018.

\bibitem{8632898}
D.~{Qin}, J.~{Yu}, G.~{Zou}, R.~{Yong}, Q.~{Zhao}, and B.~{Zhang}, ``A novel
  combined prediction scheme based on cnn and lstm for urban pm2.5
  concentration,'' \emph{IEEE Access}, pp. 1--1, 2019.

\bibitem{DBLP:conf/icml/MnihBMGLHSK16}
\BIBentryALTinterwordspacing
V.~Mnih, A.~P. Badia, M.~Mirza, A.~Graves, T.~P. Lillicrap, T.~Harley,
  D.~Silver, and K.~Kavukcuoglu, ``Asynchronous methods for deep reinforcement
  learning,'' in \emph{Proceedings of the 33nd International Conference on
  Machine Learning, {ICML} 2016, New York City, NY, USA, June 19-24, 2016},
  2016, pp. 1928--1937. [Online]. Available:
  \url{http://jmlr.org/proceedings/papers/v48/mniha16.html}
\BIBentrySTDinterwordspacing

\bibitem{DBLP:conf/infocom/XuTMZWLY18}
\BIBentryALTinterwordspacing
Z.~Xu, J.~Tang, J.~Meng, W.~Zhang, Y.~Wang, C.~H. Liu, and D.~Yang,
  ``Experience-driven networking: {A} deep reinforcement learning based
  approach,'' in \emph{2018 {IEEE} Conference on Computer Communications,
  {INFOCOM} 2018, Honolulu, HI, USA, April 16-19, 2018}, 2018, pp. 1871--1879.
  [Online]. Available: \url{https://doi.org/10.1109/INFOCOM.2018.8485853}
\BIBentrySTDinterwordspacing

\bibitem{DBLP:conf/iccv/RaoL017}
\BIBentryALTinterwordspacing
Y.~Rao, J.~Lu, and J.~Zhou, ``Attention-aware deep reinforcement learning for
  video face recognition,'' in \emph{{IEEE} International Conference on
  Computer Vision, {ICCV} 2017, Venice, Italy, October 22-29, 2017}, 2017, pp.
  3951--3960. [Online]. Available: \url{https://doi.org/10.1109/ICCV.2017.424}
\BIBentrySTDinterwordspacing

\bibitem{KDS}
Q.~Qi, J.~Wang, Z.~Ma, H.~Sun, Y.~Cao, L.~Zhang, and J.~Liao,
  ``Knowledge-driven service offloading decision for vehicular edge computing:
  A deep reinforcement learning approach,'' 2019.

\bibitem{DBLP:journals/corr/abs-1708-05144}
\BIBentryALTinterwordspacing
Y.~Wu, E.~Mansimov, S.~Liao, R.~B. Grosse, and J.~Ba, ``Scalable trust-region
  method for deep reinforcement learning using kronecker-factored
  approximation,'' \emph{CoRR}, vol. abs/1708.05144, 2017. [Online]. Available:
  \url{http://arxiv.org/abs/1708.05144}
\BIBentrySTDinterwordspacing

\bibitem{Peters+Schaal:2008-motor}
\BIBentryALTinterwordspacing
J.~Peters and S.~Schaal, ``Reinforcement learning of motor skills with policy
  gradients,'' \emph{Neural Networks}, vol.~21, no.~4, pp. 682--697, 2008.
  [Online]. Available:
  \url{http://www-clmc.usc.edu/publications/P/peters-NN2008.pdf}
\BIBentrySTDinterwordspacing

\bibitem{DBLP:journals/corr/LillicrapHPHETS15}
\BIBentryALTinterwordspacing
T.~P. Lillicrap, J.~J. Hunt, A.~Pritzel, N.~Heess, T.~Erez, Y.~Tassa,
  D.~Silver, and D.~Wierstra, ``Continuous control with deep reinforcement
  learning,'' \emph{CoRR}, vol. abs/1509.02971, 2015. [Online]. Available:
  \url{http://arxiv.org/abs/1509.02971}
\BIBentrySTDinterwordspacing

\bibitem{DBLP:journals/corr/SchulmanWDRK17}
\BIBentryALTinterwordspacing
J.~Schulman, F.~Wolski, P.~Dhariwal, A.~Radford, and O.~Klimov, ``Proximal
  policy optimization algorithms,'' \emph{CoRR}, vol. abs/1707.06347, 2017.
  [Online]. Available: \url{http://arxiv.org/abs/1707.06347}
\BIBentrySTDinterwordspacing

\bibitem{manual:Imagetext}
F.~Zhu, Z.~Ma, X.~Li, G.~Chen, J.-T. Chien, J.-H. Xue, and J.~Guo, ``Image-text
  dual model with decision strategy for small-sample image classification,'' in
  \emph{NEUROCOMPUTING}, vol. 328, 2019, pp. 182--188.

\bibitem{noauthor_image-text_nodate}
\BIBentryALTinterwordspacing
``\BIBforeignlanguage{en}{Image-text {Dual} {Neural} {Network} with {Decision}
  {Strategy} for {Small}-sample {Image} {Classification} {\textbar} {Request}
  {PDF}}.'' [Online]. Available:
  \url{https://www.researchgate.net/publication/327126961_Image-text_Dual_Neural_Network_with_Decision_Strategy_for_Small-sample_Image_Classification}
\BIBentrySTDinterwordspacing

\end{thebibliography}
